Parametric excitations of coupled nanomagnets

We demonstrate that parametrically excited eigenmodes in nearby nanomagnets can be coupled to each other. Both positive (in-phase) and negative (anti-phase) couplings can be realized by a combination of appropriately chosen geometry and excitation field frequency. The oscillations are sufficiently stable against thermal fluctuations. The phase relation between field-coupled nanomagnets shows a hysteretic behavior with the phase relation being locked over a wide frequency range. We envision that this computational study lays the groundwork to use field-coupled nanomagnets as parametrons as building blocks of logic devices, neuromorphic systems or Ising machines.

==> notes/esetleg_tovabbi_szimuk.tex <==
Fut: IR régiókkal - kimutatja-e ez is a csatolások kettős csúcsát

Fut: Hiszterézis az "alsó" csatolásokból kiindulva - azonos konstellációk különböző csatolásainak gerjesztési tartományát össze lehetne hasonlítani (negatív, vagy pozitív csatolás bírja tovább, vagy gyakorlatilag ugyanúgy viselkednek...)

Fut: Távoli mágnesekkel "léptetős" szimuláció 
    - kimutassa, hogy ez esetben nincs szép határ a csatolási tartományok között
    
(Nem priós:) Mágnes lánc IR (vagy T) régiónkénti FFT-vel - pontosabb spektrum (nem átlagolódnak ki az ellentétescsatolások)




==> notes/jegyzetek_summaries_cut.tex <==
konstelláció: hány mágnes van és egymáshoz képest milyen irányban és távolságra vannak


Korábbról: mágneses tér befolyásolja a módusok sajátfrekvenciáját

T fluktuáció nagy (300 K-en)
    25 mT amplitúdójú gerjesztést használunk a csatolásokhoz (bár 20 mT is valószínűleg elég, sokkal lejjebb nem mehetünk, ha stabil csatolásokat szeretnénk)
    20230127/11-es mérés különböző T-k jelenlétében megjelenő fluktuációt vizsgálja

pozitív-negatív csatolás amplitúdója azonos frekvencián eltérő
    (-> mert a terük másként tolja el a sajátfrekvenciájukat)

IR
    hőmérséklet kicsit kiszélesíti, de nem túlságosan
    több csúcs is van (közeli mágnespároknál bejöhet még új is az egyedüli mágneshez képest)
    mi csak az elsővel foglalkozunk (kb. uniform, hosszanti oldal menti mágnespárnál a közeli végek "visszafogják" egymást)
    mágnesek konstellációja eltolja a sajátfrekvenciákat
    
T-IR
    Csak hőmérséklettel gerjesztve is lehet spektrumot feltérképezni, sőt még talán jobban is
    mágnespár esetén az első, "fő" csúcs szétválik két külön csúcsra!
        a pozitív-negatív csatolás két külön csúcsa

Jelentős fluktuáció esetén lehet a pozitív csatolási tartományban is negatív csatolás

Default mumax solver (adaptive) értelmezhetőbb eredményeket adott mint a fix lépésközű - ezt ajánlotta a cikk is, amit küldött ebben a témában

Gerjesztő frekvencia megfelelő tartományból megválasztásával lehet kotrollálni a csatolás irányát
    rövidebb oldal menti mágnespároknál a negatív csatolás van magasabb frekvencián
    hosszabb oldal menti mágnespároknál fordítva

Frekvencia növelésével mindkét pár-konstelláció mindkét csatolásának csökken az amplitúdója

mágnes láncoknál jellemzően széleken inkább pozitív csatolás van, középen pedig inkább negatív

mágnes lánc különböző frekvenciákkal kb. ugyanakkora átlagos kitéréssel rezeg, de a pozitív/negatív csatolások száma jelentősen eltér

mágnes láncok tranziense hosszú
    2023.02.09/22-es mérés: 1500 ns környékén egy sokáig véglegesnek tűnő állapot áll be, de valahol 2600 ns után megint elkezdődik valami változás
    egyre nagyobb átlagos kitérésű "felállásokba" ugrik

nagyobb gerjesztés hathat a csatolások irányára is

A csatolások olyanok mint egyetlen mágnes módusai: ha beálltak, akkor szép lassan változtatva a frekvenciát sokkal szélesebb frekvencia tartományban gerejszthetőek és sokkal nagyobb rezgés érhető el.

A csatolások frekvencia tartománybeli szétválasztása (valószínűleg) azért lehetséges, mert a két csatolás tér módosító, ezáltal sajátfrekvencia eltoló hatása különböző, ezért a két csatolás "módusa" elmozdul egymásról.
    - a fentebbi frekvencia tartományban csak az egyik módus jöhet létre (-> fentebbi tartomány csatolása)
    - az alsó tartományban a fentebbi tartomány csatolása már nehezebben jön létre hiszterézis nélkül, viszont a másik csatolás itt hiszterézis nélkül is létrejöhet, így túlnyomórészt azzal találkozunk

1 mágnes parametrikus gerjesztése: 
    - 1 lehetséges amplitúdó + T fluktuációk varianciája
    - 2 lehetséges fázis ugyanakkora eséllyel (7/8) + némi T variancia

- Különböző távolságú mágnespárok csatolási spektruma: 
    -> A távolság növekedésével a gerjeszthető tartomány egyre közelebb kerül a különálló sajátfrekvenciához - a hosszanti mágneseknél hamarabb megközelítik, valószínűleg a konstellációból fakadóan kevésbé "beszélgetnek" a mágnesek
    -> A két csatolás tartománya összetolódik, nem feltétlenül szimmetrikusan
    -> A határ közelében lehet váltás kialakult csatolásból is, de csak az egyik irányba (a "lenti" csatolásból a "fentibe", mivel a határon az utóbbinak sokkal nagyobb amplitúdós rezgése van, ha egyszer kialakul)
    

==> notes/jegyzetek_summaries_merge.tex <==
Összefoglaló: 
	- a kódok le lettek porolva, több paraméternek meglett az ésszerű beállítása néhány sikertelen mérés után,
	- a 300 K elsőre legalábbis túl erősnek tűnik
	- hőmérséklettel, talán gyakrabban találnak bele az ellenfázisos rezgésbe, de ez nem marad fenn stabilan


Összefoglaló:
	- hőmérséklettel is lehet csatolás, bár meglepően nagy fluktuációt eredményez - ez lehet a mumax csalása is
	- magasabb hőmérsékleten (250-300K) valamivel erősebb gerjesztés kell (25mT már biztos elég)
	- magasabb hőmérsékleten kijött negatív csatolás, de egyelőre csak akkor, ha a "hőmérséklet tranziens"-t nem vártuk ki a gerjesztés bekapcsolásával
	- hőmérséklet tranziens (150 ns) kivárásával 3/3 pozitív csatolás jött ki kül. T seed-ekre


 Összefoglaló:
	- 300 K-en 20mT-val már lehet rendes gerjesztést csinálni. Kisebbel kétséges a kialakuló rezgések stabilitása.
	- "távoli" mágnesek függetlenül működnek, közeliek csatolásának működése továbbra is kérdéses
		-> ha neg. csatolás alakul ki, nagyobb a rezgés amplitúdója. Ez lehet a m.terek sajátfrek. módosítása miatt?
	- hőmérséklet kicsit kiszélesíti az IR-t, de nem túlságosan
	- 17,6-7 GHz környékén, 300K-en talán van valami?
	- készült egy egyszerű, és csúnya fázis eltérés számítás+vizualizáció


összefoglaló:
	- Ha nincs jelentős fluktuáció a mágnesezettségben, akkor úgy tűnik mindig pozitív csatolás alakul ki (5/5)
	- Ha van jelentős fluktuáció, akkor viszont van esély a negatív csatolásra, illetve az eddigiek alapján még gyakoribb is (4/5), de ez még relatíve kicsi minta
	- Felmerült ötletnek, hogy a sajátfrekvenciától kicsit eltérve talán jobban "lejthet a pálya" a negatív csatolásoknak, ezt legközelebb jó lenne kipróbálni
	- Volt egy mérés csak hőmérséklettel gerjesztve a mágneseket, ámde viszonylag hosszan (1000 ns), aminek több érdekes ereménye volt, különösen a spektrumát elemezve (13-as mérés)
	- Több különböző mérésből is úgy látszik, hogy 17,65 GHz-en is van valamilyen gerjeszthető módusa a mágneseknek (együtt és külön is)
	- Kiderült, hogy az összes mérés elején megfigyelt hatalmas begerjedés azért volt, mert a kezdeti relaxáció után lett beállítva a külső feszítő tér (így épp az ellentéte irányba fordul át a mágnesezettség)
	- A hőmérséklet jelenlétében a dinamika számítása eddig is a cikkben ajánlott solver-rel ment (az a default), de ez eltér a levélben küldöttől, majd ki kéne próbálni azt is.
	- Különböző hőmérsékletek hatása ki lett próbálva, szépen látszik az egyre nagyobb fluktuáció (11-es mérés)


Összefoglalás:
	- a fix lépésközű solver elég furcsa eredményeket adott (1-4), úgyhogy visszatértem az adaptívra
	- kicsivel a sajátfrekvencia felett, a 15,65-67 GHz-es tartományon megbízhatóan *negatív* csatolás alakult ki (5-16)
	- ezek a negatív csatolások valamivel kisebb amplitúdójú rezgések, mint a korábbiak (feltételezem azért, mert messzebb vannak a sajátfrekvenciától)
	- csak a hőmérséklettel gerjesztve szép frekvencia domént kaptam, jól látszik a sajátfrekvenciák vándorlása a mágnesek távolságának függvényében (17-24)


Összefoglaló:
	- Egy mágnes IR: nincs meg a 3. csúcs 18,55 GHz-en (ami a legutóbbi JK alapján is gyengült a mágnesek távolodásával), más jelentősebb különbség nem tűnt föl 
	- Hossztengely mentén szomszédos mágnespárok: 
		gerjesztési tartomány: 15,67 GHz - 15,81 GHz
		pozitív csatolás dominál felül
		alul volt pár negatív csatolás - több mérés kell statisztikához
		minél nagyobb frekvenica, annál kisebb rezgés amplitúdó (mindkét csatolás esetében)
		módus térbeli eloszlás: a mágnesek egymáshoz közeli végei "visszafogják" egymást, a távolabbi végek nagyobb amplitúdóval rezegnek
	- Mágnes láncok:
		egész lánc átlagos mágnesezettsége alapján nem jött ki stabil rezgés
		elég sok videó készült különböző fázisokban, amik alapján a legstabilabbnak az az állapot tűnik, amikor a lánc széleken pozitív csatolás van, középen pedig negatív
20) 15,49 GHz - 15,61 GHz
	-> 15,49 GHz-en továbbra se látszik jelentős gerjedés
	-> a másik három esetben nagyon hasonló amplitúdójú rezgés alakul ki (és van eleinte egy kisebb, kb. feleakkora) - csak mások a pozitív/negatív csatolások (ami nem meglepő különböző frekvenciás gerjesztéseknél)
	-> a harmadik esetben szinte azonnal a nagyobb amplitúdós rezgésbe váltunk
	

21) 15,515 GHz - 15,545 GHz
	-> A vizsgált intervallumok végére kialakuló rezgések nagyobb frekvenciáknál egyre kisebbek, de mindegyiknél jelentős. Elképzelhető, hogy hosszabb gerjesztések esetében a többi frekvencián is kialakulna még nagyobb amplitúdós rezgés...
	-> 20-21) alátámasztják az IR ábrát - 15,53 GHz körül van a csúcs, és tőle asszimetrikus a gerjeszthető tartomány (szélesebb a magasabb frekvenciák felé eső része)


22) 15,53 looong (3000 ns)
	-> Csak 1400 nskörül áll be a végleges (?) rezgés, tehátfeltételezhetően 20-21) szakaszai még nem a végleges stabil helyzeteket mutatták
	-> Egészen addig a rezgés amplitúdója növekszik, egyre magasabb energiájú rezgési állapotokat "talál" a lánc


Összefoglalás:
	- 50 mT-ás gerjesztéssel nem csak a rezgések amplitúdója nő meg, a kialakuló csatolások iránya is megváltozhat
	- 25 mT-s gerjesztéssel szépen elkülönül a pozitív és negatív csatolási frekvencia tartomány mindkét mágnespár konstellációban
	- a két konstellációban fordítva van a pozitív és negatív csatolási tartomány sorrendje
	- a csatolások gerjesztési tartományai nagyon hasonlóak (mindkét csatolási irányban, mindkét konstellációban): egy kezdeti nagy amplitúdós gerjedés után egyre kisebb, ahogy növeljük a frekvenciát
	- feltételezés: a gerjesztési tartományok "kiterjeszthetőek" lefelé, ha beállítjuk a csatolás irányát és fokozatosan csökkentjük a frekvenciát: mint egyetlen mágnes módusainál is
	- a lánc gerjesztés működése bonyolult :)


Összefoglalás:
	- a gerjesztési tartományok "kiterjeszthetőek" lefelé, ha beállítjuk a csatolást és fokozatosan csökkentjük a frekvenciát: mint egyetlen mágnes módusainál is
	- ez a kiterjesztés nem csak a másik csatolás tartományában teljesül, hanem tovább is - legközelebb ennek határát vizsgálom



Összefoglalás:
	- a hiszterézis tartománya sokkal szélesebb, mint a "simán" gerjeszthető tartomány
	- tudok térbeli/időbeli simítást rakni a videókra :)


==> notes/talan_bele_lehetne_meg_irni.tex <==
A mágnesek egyedül/nagyon távol 15,70 GHz-es sajátfrekvenciájúak, míg 20 nm-re 15,62-3


Csatolások háromszög alakú gerjeszthetősége; különböző csatolási irányoknál ezek egymás mellett vannak azonos irányban, csak elcsúsztatva; ezáltal a magasabb frekvenciás mindig nagyobb amplitúdó az alacsonyabb frekvenciás tartományában.


Csatolás van, mert:
    - más sajátfreki (kb. 70 MHz eltolás 20 nm távolságnál)
    - élesen elváló csat. tartományok
    - reprodukálható tartományok (határnál kérdéses)


Hőmérséklet solver "5-ös" adaptív - ezt találja ki magától is a mumax



Erősebb gerjesztéssel: 
    - az egyébként csak hiszterézissel elérhető oszcillációkból egyre több elérhető,
    - vagyis lefelé szélesedik a gerjeszthető tartomány;
    
    - a módus "csúcsánál" lévő kis amplitudós rezgések, amik gyenge gerjesztéssel elvesznek a hőmérséklet fluktuációk miatt, kierősödnek
    - vagyis valamennyit felfelé is szélesedik a gerjeszthető tartomány;

    - az erősebb gerjesztéstől nagyobb ampliúdók alakulnak ki, ez némiképp eltolhatja a tartományt?
